Adaptive Orthogonalization for Stable Estimation of the Effects of Time-Varying Treatments

Inferring the causal effects of time-varying treatments is often hindered by highly variable inverse propensity weights, particularly in settings with limited covariate overlap. Building on the key framework of Imai and Ratkovic (2015), we establish sufficient balancing conditions for identification in longitudinal studies of treatment effects and propose a novel estimator that directly targets features of counterfactual or potential covariates. Instead of balancing observed covariates, our method balances the components of covariates that are orthogonal to their history, thereby isolating the new information at each time point. This strategy directly targets the joint distribution of potential covariates and prioritizes features that are most relevant to the outcome. We prove that the resulting estimator for the mean potential outcome is consistent and asymptotically normal, even in settings where standard inverse propensity weighting fails. Extensive simulations show that our estimator attains efficiency comparable to that of g-computation while providing superior robustness to model misspecification. We apply our method to a longitudinal study of private versus public schooling in Chile, demonstrating its stability and interpretability in estimating their effects on university admission scores.

==> msm24/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> msm24/smsm01_Extensions.tex <==
%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%

\section{Extensions}\label{Extensions}

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
%\vspace{-.5cm}

\subsection{Sequential balancing}

When the optimization problem in the simultaneous approach is infeasible due to the large number of the balancing constraints, a sequential balancing approach can be applied. The sequential approach is described in the supplementary material.

% When the MSM is an additive model, the balancing constraints are motivated by 

% $\eqref{eqn::exp3} = \int \expectw{\beta_0 + g(\bar{z}_T; \beta) + \sum_{t = 1}^T\alpha_{t,\bar{z}_{t-1}}^\top x_t}f_{\omega}(\bar{X}_T(\bar{z}_{T-1}) = \bar{x}_T | \bar{Z}_T = \bar{z}_T)d\bar{x}_T = \beta_0 + g(\bar{z}_T; \beta) + \sum_{t = 1}^T\alpha_{t,\bar{z}_{t-1}}^{\top}\expectw{X_t(\bar{z}_{t-1}) | \bar{Z}_T = \bar{z}_T} = \beta_0 + \beta^\top\bar{z}_T + \sum_{t = 1}^T\alpha_{t,\bar{z}_{t-1}}^{\top}\expectw{X_t| \bar{Z}_T = \bar{z}_T}$.

% %$\eqref{eqn::exp3} = \int \expectw{\beta_0 + g(\bar{z}_T; \beta) + \sum_{t = 1}^T\alpha_{t,\bar{z}_{t-1}}^\top x_t}f_{\omega}(\bar{X}_T(\bar{z}_{T-1}) = \bar{x}_T | \bar{Z}_T = \bar{z}_T)d\bar{x}_T = \beta_0 + g(\bar{z}_T; \beta) + \sum_{t = 1}^T\alpha_{t,\bar{z}_{t-1}}^{\top}\expectw{X_t(\bar{z}_{t-1}) | \bar{Z}_T = \bar{z}_T} = \beta_0 + g(\bar{z}_T; \beta) + \sum_{t = 1}^T\alpha_{t,\bar{z}_{t-1}}^{\top}\expectw{X_t| \bar{Z}_T = \bar{z}_T}$.

% If for each $t = 1, ..., T$, each $\bar{z}_{T-1} \in \bar{\mathcal{Z}}_{T-1}$, $\expectw{X_t| \bar{Z}_{T-1} = \bar{z}_{T-1}, Z_T = 1} = \expectw{X_t| \bar{Z}_{T-1} = \bar{z}_{T-1}, Z_T = 0}$, then $\sum_{\bar{z}_{T-1} \in \bar{\mathcal{Z}}_{T-1}} \{\expectw{Y|\bar{Z}_{T-1} = \bar{z}_{T-1}, Z_T = 1}P_{\omega}(\bar{z}_{T-1}) - \expectw{Y|\bar{Z}_{T-1} = \bar{z}_{T-1}, Z_T = 0}P_{\omega}(\bar{z}_{T-1})\} = \beta_T$.

% Afterwards, if for each $t = 1, ..., T-1$, each $\bar{z}_{T-2} \in \bar{\mathcal{Z}}_{T-2}$ and $z_T \in\mathcal{Z}_{T}$, $\expectw{X_t| \bar{Z}_{T-2} = \bar{z}_{T-2}, Z_{T-1} = 1, Z_T = z_T} = \expectw{X_t| \bar{Z}_{T-2} = \bar{z}_{T-2}, Z_{T-1} = 0, Z_T = z_T}$, then \\$\sum_{\bar{z}_{T-2} \in \bar{\mathcal{Z}}_{T-2}} \sum_{z_T \in \mathcal{Z}_T}\{\expectw{Y| \bar{Z}_{T-2} = \bar{z}_{T-2}, Z_{T-1} = 1, Z_T = z_T}P_{\omega}(z_T, \bar{z}_{T-2})- \expectw{Y| \bar{Z}_{T-2} = \bar{z}_{T-2}, Z_{T-1} = 0, Z_T = z_T} P_{\omega}(z_T, \bar{z}_{T-2})\} = \beta_{T-1}$.

% Finally, if for each $\underline{z}_{2} \in \underline{\mathcal{Z}}_{2}$, $\expectw{X_1| {Z}_{1} = 1, \underline{Z}_{2} = \underline{z}_{2}} = \expectw{X_1| {Z}_{1} = 0, \underline{Z}_{2} = \underline{z}_{2}}$, then $\sum_{\underline{z}_2 \in \underline{\mathcal{Z}}_2}\{\expectw{Y|\bar{Z}_{1} = 1, \underline{z}_{2}}P_{\omega}(\underline{z}_2) - \expectw{Y|\bar{Z}_{1} = 0, \underline{z}_{2}}P_{\omega}(\underline{z}_2) \} = \beta_{1}$.

% The algorithm sequentially minimizing the weights by looping from $t = T$ to $t = 1$ and in each step solve the following optimization problem and update $\boldsymbol{w}^0$ with the product of the solution $\boldsymbol{w}$ and $\boldsymbol{w}^0$ for the next optimization problem. The starting value of $\boldsymbol{w}^0$ is uniform weights.
% \begin{align}
% \argmin_{\boldsymbol{w}} \grande\{  \sum_{i \in \mathcal{I}} w^0_i \left( w_i - \bar{w} \right)^2 : & \left|\frac{\sum\limits_{i\in \mathcal{I}_{\bar{z}_{t-1}} \cap \mathcal{I}_{z_t}} w_{i}(w^0_i\bar{X}_{itp})} 
% {\sum\limits_{i\in \mathcal{I}_{\bar{z}_{t-1}} \cap \mathcal{I}_{z_t}} w_{i}}-
% \frac{\sum\limits_{i\in \mathcal{I}_{\bar{z}_{t-1}} \cap \mathcal{I}_{z'_t}} w_{i}(w^0_i\bar{X}_{itp})}
% {\sum\limits_{i\in \mathcal{I}_{\bar{z}_{t-1}} \cap \mathcal{I}_{z'_t}} w_{i}}\right| \leq \delta_{t,p,\bar{z}_{t-1}},\nonumber \\
% \forall \bar{z}_{t-1} \in \mathcal{\bar{Z}}_{t-1}, \forall z_{t} \in \mathcal{Z}_{t}, &  p=1, ..., P; \sum\limits_{i \in \mathcal{I}_{\bar{z}_{T}}} w_{i}  =  \frac{1}{n}\left\vert{ \mathcal{I}_{\bar{z}_{T}}}\right\vert,  \forall \bar{z}_{T} \in \mathcal{\bar{Z}}_{T}; w_i \geq  0, i \in \mathcal{I} \grande\} \label{eqn::seq}
% \end{align} 

\subsection{Censoring}

Let $C_{it} = 1$ if individual $i$ is lost to follow-up at day $t$, $C_{it} = 0$ otherwise. $C_{it}$ is observed right after $X_{it}$ and $Z_{it}$. We assumed missing at random (MAR) missing mechanism, where the dependence between each variable and $C_{t}$ is only through $X_{t}$ and $Z_{t}$.

If $\bar{C}_i = (C_{i1}, C_{i2}, \cdots, C_{iT}) = \bf 0$, then $Y_{i}$ is observed. $C_{t}$ can be viewed as another time-varying treatment at time $t$ (\cite{robins2000marginal}). The assumption of sequentially ignorable censoring is
$Y(\bar{z}_T) \ci C_t| (\bar{C}_{t-1}, \bar{Z}_{t},  \bar{X}_t)$ and $X_{t+1}(\bar{z}_t) \ci C_s| (\bar{C}_{s-1}, \bar{Z}_{s}, \bar{X}_s)$, $s\leq t$. Therefore, by Assumption \ref{ignorability}a and by contraction, $Y(\bar{z}_T) \ci (Z_t, C_t)| (\bar{Z}_{t-1}, \bar{C}_{t-1}, \bar{X}_t)$; by Assumption \ref{ignorability}b, $X_{t+1}(\bar{z}_{t}) \ci (Z_s, C_s) | (\bar{Z}_{s-1}, \bar{C}_{s-1}, \bar{X}_s)$, $s\leq t$. 

The details are discussed in the supplementary materials.

% Parallel to the proof in Proposition \ref{prop1}, we have
% \begin{eqnarray}
% &&\expect{Y(\bar{z}_T)} \nonumber \\
% %&=& \int  \expect{Y(\bar{z}_T) | \bar{X}_T, \bar{Z}_T = \bar{z}_T, \bar{C}_T} f(X_T = x_T | \bar{X}_{T-1} = \bar{x}_{T-1}, \bar{Z}_{T-1} = \bar{z}_{T-1}, \bar{C}_{T-1})\nonumber \\
% %&& f(X_{T-1} = x_{T-1} | \bar{X}_{T-2} = \bar{x}_{T-2}, \bar{Z}_{T-2} = \bar{z}_{T-2}, \bar{C}_{T-2})\cdots f(X_1 = x_1)d\bar{x}_T \nonumber \\
% &=& \int  \expect{Y(\bar{z}_T) | \bar{X}_T, \bar{Z}_T = \bar{z}_T, \bar{C}_T = {\bf 0}} f(X_T = x_T | \bar{X}_{T-1} = \bar{x}_{T-1}, \bar{Z}_{T-1} = \bar{z}_{T-1}, \bar{C}_{T-1} = {\bf 0})\nonumber \\
% && f(X_{T-1} = x_{T-1} | \bar{X}_{T-2} = \bar{x}_{T-2}, \bar{Z}_{T-2} = \bar{z}_{T-2}, \bar{C}_{T-2} = {\bf 0})\cdots f(X_1 = x_1)d\bar{x}_T \nonumber \\
% && \text{\small (By sequentially ignorable assumption $Y(\bar{z}_T) \ci (Z_t, C_t)| \bar{Z}_{t-1}, \bar{C}_{t-1}, \bar{X}_t$)} \nonumber \\
% %&& \text{\small (By MAR missing mechanism)} \nonumber \\
% &=& \int  \expect{Y(\bar{z}_T)| \bar{X}_T, \bar{Z}_T = \bar{z}_T, \bar{C}_T = {\bf 0}}\nonumber \\
% && f(X_T(\bar{z}_{T-1}) = x_T | \bar{X}_{T-1}(\bar{z}_{T-2}) = \bar{x}_{T-1}, \bar{Z}_{T-1} = \bar{z}_{T-1}, \bar{C}_{T-1} = {\bf 0}) \nonumber \\
% && f(X_{T-1}(\bar{z}_{T-2}) = x_{T-1} | \bar{X}_{T-2}(\bar{z}_{T-3}) = \bar{x}_{T-2}, \bar{Z}_{T-2} = \bar{z}_{T-2}, \bar{C}_{T-2} = {\bf 0}) \cdots f(X_1 = x_1)d\bar{x}_T \nonumber \\
% && \text{\small (By the stable unit treatment value assumption (SUTVA),} \nonumber \\
% && \text{\small $Y = \sum_{\bar{z}_T \in \bar{\mathcal{Z}}_T}1\{\bar{Z}_{T} = \bar{z}_T\} Y(\bar{z}_T)$, when $\bar{C}_{T} = {\bf 0}$; $X_{t} = \sum_{\bar{z}_{t-1} \in \bar{\mathcal{Z}}_{t-1}}1\{\bar{Z}_{t-1} = \bar{z}_{t-1}\} X_{t}(\bar{z}_{t-1})$, when $\bar{C}_{t-1} = {\bf 0}$)} \nonumber \\
% &=& \int \expect{Y(\bar{z}_T)| \bar{X}_T, \bar{Z}_T = \bar{z}_T, \bar{C}_T = {\bf 0}}f(X_T(\bar{z}_{T-1}) = x_T | \bar{X}_{T-1}(\bar{z}_{T-2}) = \bar{x}_{T-1})\nonumber \\
% && f(X_{T-1}(\bar{z}_{T-2}) = x_{T-1} | \bar{X}_{T-2}(\bar{z}_{T-3}) = \bar{x}_{T-2})\cdots f(X_1 = x_1)d\bar{x}_T \nonumber \\
% && \text{\small (By $X_{t+1}(\bar{z}_{t}) \ci (Z_s, C_s) | \bar{X}_s, \bar{Z}_{s-1}, \bar{C}_{s-1}$, $s\leq t$)} \nonumber \\
% &=& \int \expect{Y(\bar{z}_T)| \bar{X}_T, \bar{Z}_T = \bar{z}_T, \bar{C}_T = {\bf 0}}f(X_T(\bar{z}_{T-1}) = x_T, \cdots, X_1 = x_1)d\bar{x}_T \nonumber \\
% &=& \int \expect{Y(\bar{z}_T)| \bar{X}_T(\bar{z}_{T-1}), \bar{Z}_T = \bar{z}_T, \bar{C}_T = {\bf 0}}f(X_T(\bar{z}_{T-1}) = x_T, \cdots, X_1 = x_1)d\bar{x}_T \label{eqn::exp22}
% \end{eqnarray}
% \begin{eqnarray}
% && \expectw{Y(\bar{z}_T)| \bar{Z}_T = \bar{z}_T, \bar{C}_T = \bf 0} \nonumber \\
% &=&  \expectw{ \expectw{Y(\bar{z}_T) | \bar{X}_T, \bar{Z}_T = \bar{z}_T, \bar{C}_T = \bf 0} | \bar{Z}_T = \bar{z}_T, \bar{C}_T = \bf 0} \nonumber \\
% && \text{\small (By the law of iterated expectation, $\expect{Y_(\bar{z}_T)}$)} \nonumber \\
% &=&  \expectw{ \expectw{Y(\bar{z}_T) | \bar{X}_T(\bar{z}_{T-1}), \bar{Z}_T = \bar{z}_T, \bar{C}_T = \bf 0} | \bar{Z}_T = \bar{z}_T, \bar{C}_T = \bf 0} \label{eqn::exp32} \\
% && \text{\small (By SUTVA)} \nonumber
% \end{eqnarray}

% If we still assume the linear structure for the potential outcome, $\expect{Y(\bar{z}_T) | \bar{X}_T(\bar{z}_{T-1}), \bar{Z}_T = \bar{z}_T, \bar{C}_T = \bf{0}} = \beta_0 + g(\bar{z}_T; \beta) + \sum_{t= 1}^T\alpha_{t,\bar{z}_{t-1}}^{\top}X_t(\bar{z}_{t-1})$, 

% $\eqref{eqn::exp22} =  {\beta_0 + g(\bar{z}_T; \beta) + \sum_{t = 1}^T \alpha_{t,\bar{z}_{t-1}}^\top \int x_t f(X_t(\bar{z}_{t-1}) = x_t | \bar{C}_{t-1} = {\bf 0}) dx_t} \\= \beta_0 + g(\bar{z}_T; \beta) + \sum_{t = 1}^T\alpha_{t,\bar{z}_{t-1}}^{\top}\expect{X_t(\bar{z}_{t-1}) | \bar{C}_{t-1} = \bf 0}$, 

% $\eqref{eqn::exp32} = \int {\expectw{\beta_0 + g(\bar{z}_T; \beta) + \sum_{t = 1}^T\alpha_{t,\bar{z}_{t-1}}^\top x_t}f_{\omega}(\bar{X}_T(\bar{z}_{T-1}) = \bar{x}_T | \bar{Z}_T = \bar{z}_T, \bar{C}_T = \bf{0})} \\ = \beta_0 + g(\bar{z}_T; \beta) +  \sum_{t = 1}^T\alpha_{t, \bar{z}_{t-1}}^{\top} \expectw{X_t | \bar{Z}_T = \bar{z}_T, \bar{C}_T = \bf{0}}$.

% If for each $t$, $\expectw{X_t | \bar{Z}_T = \bar{z}_T, \bar{C}_T = \bf{0}} = \expectw{X_t | \bar{C}_{t-1} = \bf{0}}$, then $\beta$ will be unbiasedly estimated from \eqref{eqn::exp32} by fitting a model $\expectw{Y_i|\bar{Z}_T} = g(\bar{Z}_T; \beta)$ for the weighed pseudo-population, where the weights also satisfies $P_{\omega}(\bar{z}_T|\bar{C}_T = {\bf 0}) = P(z_1)P(z_2|z_1, c_1 = 0)\cdots P(z_T|\bar{z}_{T-1}, \bar{c}_{T-1} = {\bf 0})$. Furthermore, if $\expectw{X_t | \bar{Z}_T = \bar{z}_T, \bar{C}_T = \bf{0}} = \expect{X_t(\bar{z}_{t-1})|\bar{C}_{t-1} = \bf 0}$, then $\eqref{eqn::exp22} = \eqref{eqn::exp32}$ and thus the intercept $\beta_0$ is unbiased.

% When $\alpha_{t,\bar{z}_{t-1}} = \alpha_{t}$, one proposed alternative for the target $\expect{X_t(\bar{z}_{t-1})|\bar{C}_{t-1} = {\bf 0}}$ is to find $T(\bar{X}_t, \bar{z}_{t-1}, \bar{C}_{t-1} = {\bf 0})$, such that 
% $\sum_{\bar{z}_T} \sum_{t = 1}^T\alpha_{t}^\top T(\bar{X}_t, \bar{z}_{t-1},\bar{C}_{t-1} = {\bf 0}) P_{\omega}(\bar{z}_T|\bar{C}_{T} = {\bf 0}) = \sum_{t = 1}^T \alpha_{t}^\top \expect{X_t|\bar{C}_{t-1} = {\bf 0}}$.
% Therefore, the bias in $\beta_0$ will be 

% $\sum_{\bar{z}_T}[\sum_{t = 1}^T\alpha_{t}^\top\{\expect{X_t(\bar{z}_{t-1})|\bar{C}_{t-1} = {\bf 0}} - T(\bar{X}_t, \bar{z}_{t-1}, \bar{C}_{t-1} = {\bf 0})]P_{\omega}(\bar{z}_T|\bar{C}_{T} = {\bf 0})
% \\= \sum_{t = 1}^T \alpha_{t}^\top [\sum_{\bar{z}_T}\{\expect{X_t(\bar{z}_{t-1})|\bar{C}_{t-1} = {\bf 0}} - T(\bar{X}_t, \bar{z}_{t-1}, \bar{C}_{t-1} = {\bf 0})\}P_{\omega}(\bar{z}_T|\bar{C}_{T} = {\bf 0})]\\ = \sum_{t = 1}^T\alpha_{t}^\top\{\expect{X_t(\bar{Z}_{t-1})|\bar{C}_{t-1} = {\bf 0}} - \expect{X_t|\bar{C}_{t-1} = \bf 0}\} = 0$.

% %One proposed alternative for the target $\expect{X_t(\bar{z}_{t-1}) | \bar{C}_{t-1} = \bf 0}$ is $\expect{X_t|\bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0}$, then the balancing condition becomes $\expectw{X_t | \bar{Z}_T = \bar{z}_T, \bar{C}_{t-1} = \bf 0} = \expect{X_t | \bar{z}_{t-1}, \bar{C}_T = \bf 0}$ (for any $\bar{z}_T$). 
% %The bias in the intercept will be $\sum_{\bar{z}_T}\sum_{t = 1}^T \alpha_{t,\bar{z}_{t-1}}^\top\{\expect{X_t(\bar{z}_{t-1})|\bar{C}_{t-1} = \bf 0} - \expectw{X_t | \bar{Z}_T = \bar{z}_T, \bar{C}_T = {\bf 0}}\}P_{\omega}(\bar{z}_T| \bar{C}_T = {\bf 0}) = \sum_{\bar{z}_T}\sum_{t = 1}^T\alpha_{t,\bar{z}_{t-1}}^\top\{\expect{X_t(\bar{z}_{t-1}) | \bar{C}_{t-1} = \bf 0} - \expect{X_t | \bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0}\}P_{\omega}(\bar{z}_T| \bar{C}_T = {\bf 0}) = \sum_{t = 1}^T \alpha_{t}^\top\{\expect{X_t(\bar{Z}_{t-1})|\bar{C}_{t-1} = \bf 0} - \expect{X_t|\bar{C}_{t-1} = \bf 0}\} = 0$ if $\alpha_{t,\bar{z}_{t-1}} = \alpha_{t}$.

% We have defined $V_1 := X_1$, $V_t := X_t - \sum_{k = 1}^{t-1}\eta_{t,X_{k},\bar{z}_k}X_{k}$. To achieve $ \expectw{X_t | \bar{Z}_T = \bar{z}_T,  \bar{C}_{T} = \bf{0}} = T(\bar{X}_t, \bar{z}_{t-1}, \bar{C}_{t-1} = {\bf 0})$ in the pseudo-population, we use the following constraints:

% \begin{eqnarray}
% &&\expectw{V_1|\bar{z}_T, \bar{C}_T = \bf 0} = \expect{X_1} \nonumber\\
% && \expectw{V_2|z_1, \underline{z}_2, \bar{C}_T = \bf 0} = \expect{V_2|z_1, C_1 = 0} \nonumber\\
% && \vdots \nonumber\\
% && \expectw{V_T|\bar{z}_{T-1}, z_T, \bar{C}_T = \bf 0} = \expect{V_T|\bar{z}_{T-1}, \bar{C}_{T-1} = \bf 0} \nonumber
% \end{eqnarray}

% For each strata of $\bar{z}_{t-1}$, $\eta_{t,\cdot,\cdot}$ will be estimated by regressing $X_{t+1}$ on $\bar{X}_{t}$ for the observed $X_{t+1}$. 

% \begin{proof}
% \begin{eqnarray}
% && \expectw{X_1|\bar{z}_T, \bar{C}_T = \bf 0} = \expect{X_1} \text{\small (By the balancing constraint for $X_1$)} =: T(X_1) \nonumber \\
% && \expectw{X_2|z_1, \underline{z}_2, \bar{C}_T = \bf 0}
% = \expectw{X_2 - \eta^\top_{2,X_1,z_1}X_1 | z_1, \underline{z}_2, \bar{C}_T = \bf 0} + \expectw{\eta^\top_{2,X_1,z_1} X_1| z_1, \underline{z}_2, \bar{C}_T = \bf 0}  \nonumber \\
% &=&\expect{X_2 - \eta_{2,X_1,z_1}^\top X_1 | z_1, C_1 = 0} + \eta_{2,X_1,z_1}^\top\expect{X_1} =: T(X_2, z_1, C_1 = 0)  \nonumber \\
% && \text{\small (By the balancing constraint for $X_1, X_2$)} \nonumber \\
% &&\expectw{X_t|\bar{z}_{t-1}, \underline{z}_t, \bar{C}_T = \bf 0} \nonumber \\
% &=& \expectw{X_t - \sum_{k = 1}^{t-1}\eta^\top_{t, X_k, \bar{z}_k}X_{k}|\bar{z}_{t-1}, \underline{z}_t, \bar{C}_T = \bf 0} + \expectw{\sum_{k = 1}^{t-1}\eta^\top_{t, X_k, \bar{z}_k}X_{k} | \bar{z}_{t-1}, \underline{z}_t, \bar{C}_{T} = \bf 0}  \nonumber \\
% &=&\expect{X_t - \sum_{k = 1}^{t-1}\eta^\top_{t, X_k, \bar{z}_k}X_{k}| \bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} + \expectw{\sum_{k = 1}^{t-1}\eta^\top_{t, X_k, \bar{z}_k}X_{k}| \bar{z}_{t-1}, \underline{z}_t, \bar{C}_{T} = \bf 0}  \nonumber \\
% && \text{\small (By the balancing constraint for $X_t$)} \nonumber \\
% %&=&\expect{X_t - \sum_{k = 1}^{t-1}\eta^\top_{t,X_{k},\bar{z}_k}X_{k}| \bar{z}_{t-1}, \bar{C}_{t-1} = {\bf 0}} + \sum_{k = 1}^{t-1}\eta^\top_{t,X_{k},\bar{z}_k}\expect{X_{k} | \bar{z}_{k-1}, \bar{C}_{k-1} = {\bf 0}} \nonumber \\
% &=&\expect{X_t - \sum_{k = 1}^{t-1}\eta^\top_{t,X_{k},\bar{z}_k}X_{k}| \bar{z}_{t-1}, \bar{C}_{t-1} = {\bf 0}} + \sum_{k = 2}^{t-1}\eta^\top_{t,X_{k},\bar{z}_k}\expect{X_{k}  - \sum_{j = 1}^{k-1} \eta^\top_{k,X_{j},\bar{z}_j} X_j | \bar{z}_{k-1}, \bar{C}_{k-1} = {\bf 0}} \nonumber \\
% && + \sum_{k = 1}^{t-1}\prod_{j = 1}^{k} \eta^\top_{t,X_j,\bar{z}_j}\expect{X_1} \nonumber \\
% && \text{\small (By the balancing constraint for $X_1, ..., X_{t-1}$)} \nonumber \\
% & =:& T(\bar{X}_t, \bar{z}_{t-1}, \bar{C}_{t-1} = {\bf 0}) \nonumber
% %&=&\expect{X_t - \sum_{k = 1}^{t-1}\eta_{t, X_k, \bar{z}_k}X_{k} | \bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} + \expect{\sum_{k = 1}^{t-1}\eta_{t, X_k, \bar{z}_k}X_{k}| \bar{z}_{t-1}, \bar{C}_{t-1} = {\bf 0}}  \nonumber \\
% %&& \text{\small (If $\expect{\sum_{k = 1}^{t-1}\eta_{t, X_k, \bar{z}_k}X_{k}|\bar{z}_{t-1}, \underline{z}_t, \bar{C}_{T} = \bf 0}$ does not depend on $\underline{z}_t$ and $\underline{C}_t$} \nonumber \\
% %&& \text{\small (If $\eta_{X_{t-1}}$ does not depend on $\underline{z}_t, \underline{c}_t$, by $X_{t-1} \ci (\underline{Z}_t, \underline{C}_t)| \bar{Z}_{t-1}, \bar{C}_{t-1}, X_t$. )} \nonumber \\
% %&=& \expect{X_t | \bar{z}_{t-1},\bar{C}_{t-1} = \bf 0}. \nonumber
% \end{eqnarray}

% %\begin{eqnarray}
% %&& \expect{X_1|\bar{z}_T, \bar{C}_T = \bf 0} = \expect{X_1} \nonumber \\
% %&&\expect{X_t|\bar{z}_{t-1}, \underline{z}_t, \bar{C}_T = \bf 0} \nonumber \\
% %&=& \expect{X_t - \expect{X_t|X_{t-1}, \bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} + \expect{X_t|X_{t-1}, \bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0}|\bar{z}_{t-1}, \underline{z}_t, \bar{C}_{t-1} = \bf 0} \nonumber \\
% %&=& \expect{X_t - \eta_{X_{t-1}}\expect{X_{t-1}|\bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} | \bar{z}_{t-1}, \underline{z}_t, \bar{C}_T = \bf 0} \nonumber \\
% %&+& \expect{\eta_{X_{t-1}}\expect{X_{t-1}|\bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} | \bar{z}_{t-1}, \underline{z}_t, \bar{C}_{T} = \bf 0}  \nonumber \\
% %&=&\expect{X_t - \eta_{X_{t-1}}\expect{X_{t-1}|\bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} | \bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0}  \nonumber \\
% %&+& \expect{\eta_{X_{t-1}}\expect{X_{t-1}|\bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} | \bar{z}_{t-1}, \underline{z}_t, \bar{C}_{T} = \bf 0}  \text{    \small (By the t-th constraint for $X_t$)}  \nonumber \\
% %&=&\expect{X_t - \eta_{X_{t-1}}\expect{X_{t-1}|\bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} | \bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} \nonumber \\
% %&+& \expect{\eta_{X_{t-1}}\expect{X_{t-1}|\bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} | \bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0}  \nonumber \\
% %&& \text{\small (If $\eta_{X_{t-1}}$ does not depend on $\underline{z}_t, \underline{c}_t$, by $X_{t-1} \ci (\underline{Z}_t, \underline{C}_t)| \bar{Z}_{t-1}, \bar{C}_{t-1}, X_t$. )} \nonumber \\
% %&=&\expect{X_t - \zeta(\bar{z}_{t-1}) - \eta_{X_{t-1}}\expect{X_{t-1}|\bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} | \bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} + \zeta(\bar{z}_{t-1}) \nonumber \\
% %%&+& \expect{\eta_{X_{t-1}}\expect{X_{t-1}|\bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} | \bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0}  \nonumber \\
% %&=&\expect{X_t - \zeta(\bar{z}_{t-1}) - \eta_{X_{t-1}}\expect{X_{t-1}|\bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} | \bar{C}_{t-1} = \bf 0} + \zeta(\bar{z}_{t-1}) \nonumber \\
% %&+& \expect{\eta_{X_{t-1}}\expect{X_{t-1}|\bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} | \bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0}  \nonumber \\
% %&& \text{\small (If $X_t - \zeta(\bar{z}_{t-1}) - \eta_{X_{t-1}}\expect{X_{t-1} | \bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0}$ does not depend on $\bar{z}_{t-1}$ conditioning on $\bar{C}_{t-1}$)} \nonumber \\
% %&=&\expect{X_t - \zeta(\bar{z}_{t-1}) - \eta_{X_{t-1}}\expect{X_{t-1}|\bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} | \bar{C}_{t-1} = \bf 0} + \zeta(\bar{z}_{t-1}) \nonumber \\
% %&+& \expect{\eta_{X_{t-1}}\expect{X_{t-1}|\bar{z}_{t-1}, \bar{C}_{t-1} = \bf 0} | \bar{C}_{t-1} = \bf 0} \nonumber \\
% %&& \text{\small (If $\eta_{X_{t-1}}$ does not depend on $\bar{z}_{t-1}$ when conditioning on $\bar{C}_{t-1}$)} \nonumber \\
% %&=& \expect{X_t | \bar{C}_{t-1} = \bf 0}. \nonumber
% %\end{eqnarray}
% \end{proof}

% The optimal weights are given by

% \begin{align*}
% &\argmin_{\boldsymbol{w}} \grande\{  \sum_{i \in \mathcal{I}_T} \left( w_i - \bar{w} \right)^2 :  \left|\frac{\sum\limits_{i\in \mathcal{I}_{\bar{z}_{t-1}} \cap \mathcal{I}_{\underline{z}_t}} w_{i}V_{itp}} 
% {\sum\limits_{i\in \mathcal{I}_{\bar{z}_{t-1}} \cap \mathcal{I}_{\underline{z}_t}} w_{i}}-
% \frac{\sum\limits_{i\in \mathcal{I}_{\bar{z}_{t-1}} }V_{itp}}
% {\left\vert{ \mathcal{I}_{\bar{z}_{t-1}}}\right\vert}\right| \leq \delta_{t,p,\bar{z}_{t-1}}, \forall \bar{z}_{t-1} \in \mathcal{\bar{Z}}_{t-1}, \forall \underline{z}_{t} \in \mathcal{\underline{Z}}_{t},\\
% & t=1...,T, p=1,...,P; \sum\limits_{i \in \mathcal{I}_{\bar{z}_{T}} \cap \mathcal{I}_T} w_{i}  =  \frac{1}{n}\left\vert{ \mathcal{I}_{\bar{z}_{T}} \cap \mathcal{I}_T}\right\vert\frac{\prod_{t= 1}^T\left\vert{ \mathcal{I}_{\bar{z}_{t}}}\right\vert}{\prod_{t= 1}^T \left\vert{ \mathcal{I}_{\bar{z}_{t}} \cap \mathcal{I}_t}\right\vert},  \forall \bar{z}_{T} \in \mathcal{\bar{Z}}_{T}; w_i \geq  0, i \in \mathcal{I}_T \grande\}
% \end{align*}  

% \noindent
% where $V_{itp} = X_{itp} - \sum_{k = 1}^{t-1}\hat{\eta}_{t,X_{k}, \bar{z}_{k}, p}^\top X_{i(t-1)}$, $\mathcal{I}_t = \{i: \bar{C}_{it} = {\bf 0}, ~ i \in 1,...,n \}$, $\mathcal{I}_{\bar{z}_t}=\{i \in \mathcal{I}_{t-1} : \bar{Z}_{it}=\bar{z}_t\}$, $\mathcal{I}_{\underline{z}_t}=\{i \in \mathcal{I}_T : \underline{Z}_{it}=\underline{z}_t\}$, ${X}_{itp}$ is covariate $p$ at time $t$ for subject $i$, and $\delta_{t,p,\bar{z}_{t-1}}$ is a scalar determined by the investigator. 

% The equal constrains have the above form because of

% $P_{\omega}(\bar{z}_T|\bar{C}_T = {\bf 0}) = P(z_1)P(z_2|z_1, C_1 = 0)\cdots P(z_T|\bar{z}_{T-1}, \bar{C}_{T-1} = {\bf 0}) \\
% = P(z_1)\frac{P(C_1 = 0|z_1)}{P(C_1 = 0|z_1)}P(z_2|z_1, c_1 = 0)\frac{P(C_2 = 0|\bar{z}_2, C_1 = 0)}{P(C_2 = 0|\bar{z}_2, C_1 = 0)}\cdots P(z_T|\bar{z}_{T-1}, \bar{C}_{T-1} = {\bf 0})\frac{P(C_{T-1} = 0|\bar{z}_{T-1}, \bar{C}_{T-2} = 0)}{P(C_{T-1} = {\bf 0}|\bar{z}_{T-1}, \bar{C}_{T-2} = {\bf 0})} \\ = \frac{P(\bar{z}_T, \bar{C}_{T-1})P(C_{T} = {\bf 0}|\bar{z}_{T}, \bar{C}_{T-1} = {\bf 0})}{P(C_1 = 0| z_1)P(C_2 = 0|\bar{z}_2, C_1 = 0)\cdots P(C_{T-1} = 0|\bar{z}_{T-1}, \bar{C}_{T-2} = {\bf 0})P(C_{T} = 0|\bar{z}_{T}, \bar{C}_{T-1} = {\bf 0})} \\ = \frac{P(\bar{z}_T,\bar{C}_{T} = {\bf 0})}{\prod_{t = 1}^TP(C_{t} = 0|\bar{z}_{t}, \bar{C}_{t-1} = 0)}$.


